MetaHTR: Towards Writer-Adaptive Handwritten Text Recognition

Handwritten Text Recognition (HTR) remains a challenging problem to date, largely due to the varying writing styles that exist amongst us. Prior works however generally operate with the assumption that there is a limited number of styles, most of which have already been captured by existing datasets. In this paper, we take a completely different perspective -- we work on the assumption that there is always a new style that is drastically different, and that we will only have very limited data during testing to perform adaptation. This results in a commercially viable solution -- the model has the best shot at adaptation being exposed to the new style, and the few samples nature makes it practical to implement. We achieve this via a novel meta-learning framework which exploits additional new-writer data through a support set, and outputs a writer-adapted model via single gradient step update, all during inference. We discover and leverage on the important insight that there exists few key characters per writer that exhibit relatively larger style discrepancies. For that, we additionally propose to meta-learn instance specific weights for a character-wise cross-entropy loss, which is specifically designed to work with the sequential nature of text data. Our writer-adaptive MetaHTR framework can be easily implemented on the top of most state-of-the-art HTR models. Experiments show an average performance gain of 5-7% can be obtained by observing very few new style data. We further demonstrate via a set of ablative studies the advantage of our meta design when compared with alternative adaption mechanisms.

==> argument.tex <==
removing $g_\gamma$ from our model makes it similar to MAML. Hence its value should be exactly same as that of MAML. A GAP of 2.1\%

removing $\mathcal{L}_c(\theta)$ from equation 4 drops performance by 1.3\%. Hence, it means that contribution by combined $\mathcal{L}_{ce}^{t}$ and $\mathcal{L}_c$ is much more than $\mathcal{L}_{ce}^{t}$ alone.

not using learnable learning rate drops performance by 0.6\%, 0.5\%, 0.5\% for ASTER, SAR and SCATTER. While this shows that having instance-weighting is more important than using learnable learning rate. i.e. I would rather use instance-weighting mechanism than choose learnable learning rate.

==> pinaki-backup.tex <==
\begin{table*}
\centering
\caption{Comparison of the proposed method with existing text recognition techniques in the past few years.}
\resizebox{2.\columnwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|l}
\hline\hline
\textbf{Methods} & \textbf{Year}  & \textbf{IIIT-5K} & \textbf{SVT} & \textbf{IC13} & \textbf{IC15} & \textbf{SVT-P} & \textbf{CUTE80} & \textbf{Remarks} \\
\hline
    Shi \etal \cite{Shi2015} & 2015 & 81.2 & 82.7 & 89.6 & - & 66.8 & 54.9 & End-to-end trainable CNN + RNN + CTC framework \\
    \hline
    Lee and Osindero \cite{lee2016recursive} & 2016 & 78.4 & 80.7 & - & 90.8 & - & 42.7 & Recursive CNN + RNN for LM + Soft Atten. decoder \\
    Shi \etal \cite{shi2016rare} & 2016 & 81.9 & 81.9 & 88.6 & - & - & - & Spatial Transformer Network(STN) + CNN + RNN + Atten. decoder \\
    \hline
    Cheng \etal \cite{cheng2017focusing} & 2017 & 87.4 & 85.9 & 93.3 & 70.6 & 71.5 & 63.9 & Char. annot. + Atten. drift + CNN-RNN-Atten. decoder \\
    \hline
    Liu \etal \cite{liu2018charnet} & 2018 & 83.6 & 84.4 & - & 60.0 & 73.5 & - & Char. annot. + CNN + Hierarchial Atten. Mechanism + LSTM-decoder \\
    Bai \etal \cite{bai2018edit} & 2018 & 88.3 & 87.5 & 94.4 & 73.9 & - & - & Char. annot. + CNN + RNN + Edit Prob. based Atten. decoder \\
    Liu \etal \cite{liu2018feature} & 2018 & 89.4 & 87.1 & 94.0 & - & 73.9 & 62.5 & Char. annot. + CNN + bLSTM + CTC + GAN \\
    Shi \etal \cite{shi2018aster} & 2018 & 93.4 & 93.6 & 91.8 & 76.1 & 78.5 & 79.5 & Thin Plate Spline(TPS) Img. rectification + CNN-RNN-Atten. decoder \\
    Cheng \etal \cite{cheng2018aon} & 2018 & 87.0 & 82.8 & - & 68.2 & 73.0 & 76.8 & CNN + 4 directional Atten. + bLSTM + Atten. decoder \\
    \hline
    Liao \etal \cite{liao2019scene} & 2019 & 91.9 & 86.4 & 91.5 & - & - & 79.9 & Char. Atten. FCN with pixel classification in 2D fashion \\
    % Liao \etal \cite{liao2019maskTextspotter} & 2019 & 95.3 & 91.8 & 95.3 & 78.2 & 83.6 & 88.5 \\
    Yang \etal \cite{yang2019symmetry} & 2019 & 94.4 & 88.9 & 93.9 & 78.7 & 80.8 & 87.5 & Geometrical attributes + TPS for rectification + CNN-RNN-Atten. decoder \\
    Luo \etal \cite{moran} & 2019 & 91.2 & 88.3 & 92.4 & 68.8 & 76.1 & 77.4 & Geometric constraints Free STN + CNN + bLSTM + Fractional Pickup + Atten. decoder \\
    Li \etal \cite{li2019show} & 2019 & 95.0 & 91.2 & 94.0 & 78.8 & 86.4 & 89.6 & CNN + bLSTM + 2D Atten. decoder\\
    Baek \etal \cite{baek2019wrong} & 2019 & 87.9 & 87.5 & 92.3 & 71.8 & 79.2 & 74.0 & holistic \& fair comparison of STR method; 4-stage generalised framework for STR \\
    Zhan \etal \cite{ESIR2019} & 2019 & 93.3 & 90.2 & 91.3 & 76.9 & 79.6 & 83.3 & Iterative Image rectification + CNN-RNN-Atten. decoder \\
    \hline
    Litman \etal \cite{litman2020scatter} & 2020 & 93.7 & 92.7 & 93.9 & 82.2 & 86.9 & 87.5 & Img. rectification + CNN + bLSTM + Visual Feature Refine + Selective-Decoder \\
    Qiao \etal \cite{qiao2020seed} & 2020 & 93.8 & 89.6 & 92.8 & 80.0 & 81.4 & 83.6 & Img. rectification + CNN + bLSTM + Global Semantic info. from LM + Atten. decoder \\
    Yu \etal \cite{yu2020towards} & 2020 & 94.8 & 91.5 & 95.5 & 82.7 & 85.1 & 87.8 & CNN+Parallel Visual Atten.+Global Semantic Reasoning+Visual-Semantic Fusion Decoder \\
    \hline
    Proposed Method & 2021 & xxx & xxx & xxx & xxx & xxx & xxx \\
    \hline
\end{tabular}}
\end{table*}




\setlength{\tabcolsep}{4.5pt}
\begin{table*}
	\begin{minipage}{0.6\linewidth}
		\caption{hello}
		\label{table:student}
		\centering
		\scriptsize
            \begin{tabular}{c|cc|cc|ccc|cc|cc|ccc}
            \Xhline{2\arrayrulewidth}
             &  \multicolumn{7}{c|}{{IAM} \cite{marti2002iam} (WRA)} & \multicolumn{7}{c}{{RIMES} \cite{augustin2006rimes} (WRA)}\\
             \cline{2-15}
            Methods & \multicolumn{2}{c|} {{Baseline}} & \multicolumn{2}{c|} {{Fine-tuning}} &\multicolumn{3}{c|}{{MetaHTR}}&  \multicolumn{2}{c|}{{Baseline}} & \multicolumn{2}{c|} {{Fine-tuning}} & \multicolumn{3}{c}{{MetaHTR}}\\
            \cline{2-15}
            %  \textbf{} & \multicolumn{2}{c|}{WRA} & \multicolumn{2}{c|}{WRA} & \multicolumn{3}{c|}{WRA} & \multicolumn{2}{c|}{{WRA}} & \multicolumn{2}{c|}{WRA} & \multicolumn{3}{c}{WRA} \\
             & L & None & L & None & L & None & GAP & L & None & L & None & L & None & GAP \\
             \hline
                ASTER \cite{shi2018aster} & 90.3 & 81.3 & 90.5 & 81.7 & 94.1 & 89.2 & 7.9 & 93.6 & 87.4 & 93.7 & 87.7 & 96.5 & 93.4 & 6.0 \\
                \hline
                SAR \cite{li2019show}  & 91.6 & 84.4 & 91.7 & 84.7 & 94.8 & 91.5 & 7.1 & 93.8 & 88.7 & 93.8 & 88.8 & 96.5 & 93.7 & 5.0 \\
                \hline
                SCATTER \cite{litman2020scatter} & 91.7 & 84.6 & 92.0 & 85.1 & 94.8 & 91.6 & 7.0 & 93.8 & 88.8 & 93.9 & 89.0 & 96.6 & 93.9 & 5.1 \\
                \hline
            \end{tabular}
	\end{minipage}\hfill
	\begin{minipage}{0.23\linewidth}
		\centering
		\includegraphics[width=4.0cm, height=2.6cm]{latex/metaHTRvsMAML2.pdf}
% 		\label{ }
	\end{minipage}
	\vspace{-0.6cm}
\end{table*}
